Detecting long-lived particles trapped in detector material at the LHC

We propose to implement a two-stage detection strategy for exotic long-lived particles that could be produced at the CERN LHC, become trapped in detector material, and decay later. The proposed strategy relies on an array of metal rods, combined to form a high-density target. In a first stage, the rods are exposed to radiation from LHC collisions in one of the experimental caverns. In a second stage, they are individually immersed in liquid argon in a different experimental hall, where out-of-time decays could produce a detectable signal. Using a benchmark case of long-lived gluino pair production, we show that this experiment would be sensitive to a wide range of masses. Such an experiment would have unique sensitivity to gluino-neutralino mass splittings down to 3 GeV, in previously uncovered particle lifetimes ranging from days to years.

==> prlJustification.tex <==
%a short justification (less than 100 words) describing how the Letter substantially advances the field, opens a significant new area of research, solves (or makes a significant step towards solving) a critical outstanding problem, or is otherwise of great general interest. It is also important that the authors state that the analysis addresses a sufficiently original and timely physics topic (otherwise it should be published as a regular article rather than as a letter).
%importance, broad interest

This work proposes a novel experiment and an original detection strategy to probe the existence of LLPs, which are of significant and growing interest to high-energy physics and can arise in many BSM scenarios. This proposal is timely, with the upcoming LHC Run 3 and the HL-LHC. The strategy is advantageous because it includes a compact, movable target, which could be adapted to cover different acceptances during exposure campaigns targeting different BSM scenarios. This experiment would have unique sensitivity to mass splittings down to 3~GeV and probe very long lifetimes, which are the most challenging for traditional techniques at colliders.
